Findings of the NLP4IF-2021 Shared Tasks on Fighting the COVID-19 Infodemic and Censorship Detection

We present the results and the main findings of the NLP4IF-2021 shared tasks. Task 1 focused on fighting the COVID-19 infodemic in social media, and it was offered in Arabic, Bulgarian, and English. Given a tweet, it asked to predict whether that tweet contains a verifiable claim, and if so, whether it is likely to be false, is of general interest, is likely to be harmful, and is worthy of manual fact-checking; also, whether it is harmful to society, and whether it requires the attention of policy makers. Task~2 focused on censorship detection, and was offered in Chinese. A total of ten teams submitted systems for task 1, and one team participated in task 2; nine teams also submitted a system description paper. Here, we present the tasks, analyze the results, and discuss the system submissions and the methods they used. Most submissions achieved sizable improvements over several baselines, and the best systems used pre-trained Transformers and ensembles. The data, the scorers and the leaderboards for the tasks are available at http://gitlab.com/NLP4IF/nlp4if-2021.

==> sections/participants_systems.tex <==
\section{Participating Systems}
\label{sec:participants_systems}


\subsection{Task 1: COVID-19 Infodemic}
\todo[inline]{TODO: write --> Firoj}

Team \textbf{Damascus}~\cite{NLP4IF-2021-DamascusTeam} 
used an approach based on the AraBERT model. It is in the form of a two-step pipeline, where the first step involves a series of pre-processing procedures to transform Twitter jargon, including emojis and emoticons, into plain text. In the second step a version of AraBERT was exploited to fine-tune and classify the tweets. The system ranked 5th on the Arabic dataset.

Team \textbf{NARNIA}~\cite{NLP4IF-2021-NARNIATeam} 
presents work aims at identifying tweets regarding COVID19, which contains harmful and false information. We have experimented with a number of Deep Learning based models, including different word embeddings, such as Glove, ELMo, among others. BERTweet model achieved the best overall F1-score of 0.881 and secured the third rank on the above task.

Team \textbf{R00}~\cite{NLP4IF-2021-R00Team}
had the best performing system for the Arabic subtask. It used an ensemble of neural networks combining a linear layer on top of one out of the following four pre-trained Arabic language models: AraBERT, Asafaya-BERT, ARBERT, MARBERT. 

Team \textbf{dunder\_mifflin}~\cite{NLP4IF-2021-DunderMifflinTeam}
built a multi-output model using task-wise multi-head attention for inter-task information aggregation. This was built on top of the Bidirectional Encoder Representations obtained from the RoBERTa Transformer. To tackle the small size of the dataset back-translation was used for data augmentation. The loss-function was weighted for each output, in accordance with the distribution of labels for that output. They were the runners-up in the English subtask with a mean F1-score of 0.891 on the test set, without the use of any task-specific embeddings or ensembles.

Team \textbf{iCompass}~\cite{NLP4IF-2021-iCompassTeam} 
used state-of-the-art contextualized text representation models that were fine-tuned for the down-stream task in hand. ARBERT, MARBERT,AraBERT, Arabic ALBERT  and BERT-base-arabic were used. According to the results, BERT-base-arabic had the highest 0.748 F1 score on the test set.

Team \textbf{TOKOFOU}~\cite{NLP4IF-2021-TOKOFOUTeam} 
gathered a collection of 6 BERT-based language models trained in domains (e.g., Twitter and COVID-themed data), or fine-tuned on tasks similar to the shared task’s topic (e.g., hate speech and sarcasm detection). Every model was then finetuned on the shared task data, projecting a label from the sequence classification token for each of the 7 questions in parallel. After carrying out model selection on the basis of development set F1 performance, the team cast the models into a majority based ensemble to counteract the small size of the dataset and ensure robustness.

Team \textbf{HunterSpeechLab}~\cite{NLP4IF-2021-HunterSpeechLabTeam}
explored the cross-lingual generalization ability of multitask models trained from scratch (logistic regression, transformer encoder) and pre-trained models (En- glish BERT, m-BERT) for deception detection 

Team \textbf{InfoMiner}~\cite{NLP4IF-2021-InfoMinerTeam}
participated in all three languages of the task. They used pre-trained transformer models, specifically BERT base cased, RoBERTa base, BERT multilingual cased and AraBERT. They optimised the transformer models for each question separately and used undersampling to deal with the imbalancement of the data. They achieved 4th place in all the languages.


\subsection{Task 2: Censorship Detection}

